Warp Bridge Sampling: The Next Generation

Bridge sampling is an effective Monte Carlo method for estimating the ratio of normalizing constants of two probability densities, a routine computational problem in statistics, physics, chemistry, and other fields. The Monte Carlo error of the bridge sampling estimator is determined by the amount of overlap between the two densities. In the case of uni-modal densities, Warp-I, II, and III transformations (Meng and Schilling, 2002) are effective for increasing the initial overlap, but they are less so for multi-modal densities. This paper introduces Warp-U transformations that aim to transform multi-modal densities into Uni-modal ones without altering their normalizing constants. The construction of a Warp-U transformation starts with a Normal (or other convenient) mixture distribution $\phi_{\text{mix}}$ that has reasonable overlap with the target density $p$, whose normalizing constant is unknown. The stochastic transformation that maps $\phi_{\text{mix}}$ back to its generating distribution $N(0,1)$ is then applied to $p$ yielding its Warp-U version, which we denote $\tilde{p}$. Typically, $\tilde{p}$ is uni-modal and has substantially increased overlap with $N(0,1)$. Furthermore, we prove that the overlap between $\tilde{p}$ and $N(0,1)$ is guaranteed to be no less than the overlap between $p$ and $\phi_{\text{mix}}$, in terms of any $f$-divergence. We propose a computationally efficient method to find an appropriate $\phi_{\text{mix}}$, and a simple but effective approach to remove the bias which results from estimating the normalizing constants and fitting $\phi_{\text{mix}}$ with the same data. We illustrate our findings using 10 and 50 dimensional highly irregular multi-modal densities, and demonstrate how Warp-U sampling can be used to improve the final estimation step of the Generalized Wang-Landau algorithm (Liang, 2005), a powerful sampling and estimation method.

==> sec5.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Warp-U extension of Generalized Wang-Landau method}\label{sec:comparison}

%Whereas the theorericalSo far we have considered the scenario in which we have $n$ i.i.d. samples $\omega_1,\dots,\omega_n \overset{}{\sim} p$ at our disposal. In practice, the samples may instead be correlated samples obtained via one of the many Markov chain MC (MCMC) methods available, such as Metropolis-Hastings, Hamiltonian MC, or parallel tempering. However, the correlation between samples can be substantially reduced by thinning, i.e., running the MCMC algorithm for multiple steps between each recorded sample. Thus, the methods described so far also apply when MCMC algorithms are used to obtain samples from $p$. %Thinning to obtain approximately independent samples is required by many MC estimation approaches and so is not a disadvantage of (warp) bridge sampling. %Many MC estimation approaches rely on independent samples from the target so thinning is not a disadvantage of bridge sampling and warp would not be %The impact of correlation can also be accounted for by computing an effective sample size $n_{eff}$ to use in place of $n$ in the bridge sampling estimator, {\color{red} see \dots XL?}

As we emphasized earlier, bridge sampling is applicable to general MCMC settings. We therefore do not need the draws to be independent, as long as they are from the target $p$, or at least in the long run.
There are cases, however, where  the available draws are from a distribution that is known to be different from the target $p$. Indeed, some of the most promising approaches for estimating normalizing constants combine the tasks of sampling and estimation into one coherent algorithm, but often do not directly sample from $p$.  %Many of these combined approaches are forms of the adaptive importance sampling methods mentioned in Section \ref{sec:introduction}. The success of combined sampling and estimation algorithms is intuitive in the sense that an algorithm which uses the current estimation performance to inform future sampling should produce better estimates than approaches which complete all the sampling first and only then consider estimation.
An important case of such a combined approach is the generalized Wang-Landau (GWL) algorithm proposed by \citet{liang2005generalized}. GWL is particularly useful in the current context because of its ability to efficiently sample from highly multi-modal distributions.  We therefore take it as a benchmark, and illustrate how it can be combined with Warp-U bridging sampling to obtain an improved estimator for normalizing constants. More generally,  our strategy of incorporating a Warp-U bridge sampling step can be tried on other algorithms that combine sampling and estimation of normalizing constants. %can be combined with other similar algorithms to offer in a similarly improve the estimatother algorithms%to compare against. The comparison is not direct because our proposed method only regards how to {\it use} samples once they are obtained, and says nothing about how to obtain samples in the first place.\footnote{{\color{red}However, future work is to investigate the potential gains to be made by applying Warp-U in sampling algorithms, see Section \ref{sec:sampling} and Appendix \dots for discussion of this idea.}}  Nonetheless, we will see that there is a substantial benefit to integrating  our Warp-U bridge sampling method into GWL, and it is likely that Warp-U can improve other algorithms in a very similar way.


\subsection{GWL algorithm}\label{sec:gwl}

We begin by briefly describing GWL, which shares some similarities with other energy based methods such as the equi-energy sampler  \citep{kou2006equi}. Suppose that we want to compute the integral $\int_Sq(\omega)\measure(\ud\omega)$, for some unnormalized density $q$ and bounded region $S$. Typically $S$ is the region over which $q$ has non-negligible density, i.e.,  $q(S)\approx 1$.  We divide $S$ into $r$ subregions $S_1,\dots,S_r$, which are defined by target energy bins; that is, within each
$S_i$, the energy level, defined by $-\log q$,  is roughly the same. %Sampling is then performed using a modified Metropolis--Hastings algorithm.
Let the current estimate of the integral $\int_{S_i} q(\omega)\measure(\ud\omega)$ be denoted by $\hat{g}(S_i)$, and set the initial estimate to be $\hat{g}(S_i)=1$, for $i=1,\dots,r$. %Each time the subregion $E_i$ is sampled a small constant $\delta$ is added to the estimate  $\hat{g}(S_i)$.
GWL takes the inputs $n_0$, $\delta_0$, and $T$ (e.g., $n_0=1000$, $\delta_0=e-1\approx 1.718$, $T=25$) and proceeds as detailed below. Note that, \citet{liang2005generalized} introduces an additional tuning parameter, which is not needed when the goal is to estimate normalizing constants, and therefore it is not included here.
\vspace{0.2cm}

\noindent {\bf GWL algorithm.}\\
\noindent For stage $t=1,\dots,T$:
\vspace{-\topsep}
\begin{enumerate}
\setlength{\itemsep}{-0.3cm}
    \item Set $n_t=n_{t-1}(1.1)^{t-1}$, $\delta_t=\sqrt{1+\delta_{t-1}}-1$, and $\hat{g}(S_i)^{(t,1)}=\hat{g}(S_i)^{(t-1,n_{t-1})}$, for $i=1,\dots,r$.
    \item For $k=1,\dots, n_t$ do the following:
    \vspace{-\topsep}
    \begin{enumerate}[(i)]
    \setlength{\itemsep}{-0.3cm}
     \setlength{\topskip}{-2cm}
    \item Use a Metropolis-Hastings step, with proposal density $h$, to
draw a sample $\omega$ from
    the current target density
    \vspace{-0.3cm}
    \begin{align}
        \psi^{(t,k)}(\omega) \propto \sum_{i=1}^r \frac{q(\omega)}{\hat{g}^{(t,k)}(S_i)}I(\omega\in S_i).\label{eqn:intermediate}
    \end{align}
    The $(t,k)$ superscripts indicate that the current target and the estimate of $g(S_i)$, for $i=1,\dots,r$, are updated in each iteration within each stage.\\
\item Update $\hat{g}^{(t,k)}(S_{I_\omega})$ to $(1+\delta_t)\hat{g}^{(t,k)}(S_{I_\omega})$, where $I_\omega$ is the index such that $\omega \in S_{I_\omega}$, i.e., a regional mass estimate $\hat{g}^{(t,k)}(S_i)$ is increased only if $S_i$ contains the draw $\omega$.
\end{enumerate}
\end{enumerate}%Since sampling can in theory continue indefinitely, the estimates $\hat{g}(S_i)$ continue to increase and are only determined up to a common constant $c$ (which changes with the number of Metropolis--Hastings iterations). However, there is a way to estimate $c$, which we discuss in the next paragraph. Moving on,
%For simplicity suppose the proposal density is symmetric. Then, %letting $I_x$ be such that $x\in S_{I_x}$,
%if the current sample $\omega$ is in subregion $S_{I_\omega}$, the acceptance probability of a new sample $\omega^*$ in subregion $S_{I_{\omega^*}}$ is given by $\min\left\{\frac{\hat{g}(S_{I_\omega})p(\omega^*)}{\hat{g}(S_{I_{\omega^*}})p(\omega)},1\right\}$.
%The approach in \citet{liang2005generalized} is to run this algorithm in multiple stages, where each new stage corresponds to a decrease in $\delta$ and an increase in the number of iterations. This method leads

It should be clear from the description above that, in the limit, GWL samples the subregions $S_1, \ldots, S_r$ with equal probability, and within each $S_i$, it samples according to $q$. Therefore its stationary distribution is not the targeted $q$, but what can intuitively be described as a ``re-distributed" $q$ that equalizes the masses of the energy bins:
\begin{equation}
\psi(\omega)=\sum_{i=1}^r \frac{q(\omega)}{g(S_i)}I(\omega\in S_i).
\end{equation}
\citet{liang2005generalized} verified this convergence assuming that the intermediate densities of (\ref{eqn:intermediate}) can be sampled from exactly. Practically, we can sample from them approximately, say by repeating the Metropolis-Hastings step many times between each update of the estimate of $g(S_i)$, for $i=1,\dots,r$. However, \citet{liang2005generalized} used only one Metropolis-Hastings update in his illustrations, and we follow this practice (but with an ideal proposal, see Appendix \ref{app:gwl_details}). His proof also assumed $n_t$ grows sufficiently fast with $t$, but the multiplicative factor $1.1$ suggested in  \citet{liang2005generalized} may not always be adequately large, though it seems computationally problematic to increase it much further.

Since GWL samples the subregions uniformly, the final estimators $\hat{g}(S_i)=\hat{g}^{(T,n_T)}(S_i)$  estimate the integrals $g(S_i)$ only up to a common constant, denoted $A$, which depends on $\delta_0$ and the number of iterations made at each stage of the algorithm. To estimate the log normalizing constant of $q$, namely $\lambda=\log(c)$, we must remove $A$, which can be done by running GWL with a modified version of $q$ as we now explain. Choose $S_2,\dots,S_r$ to be such that $\left(\bigcup_{i=2}^rS_i\right)^c$ has negligible mass under $q$, and choose $S_1 \subset \left(\bigcup_{i=2}^rS_i\right)^c$ such that its volume $|S_1|$ is finite and known \citep{liang2005generalized}. Next, run GWL with $q$ replaced by
\begin{align*}
    q_{\text{mod}}(\omega) = \left\{\begin{array}{cc}q(\omega) & \mbox{for } \omega \in \bigcup_{i=2}^rS_i\\
    \frac{1}{|S_1|} & \mbox{for }\omega\in S_1\\
    0 & \mbox{otherwise.}\end{array}\right.
\end{align*}
The basic idea is that on $S_1$ we can treat $q$ as uniform since its actual distribution contributes little to the normalizing constant of $q$.
Lastly, for each $S\in\{S_2,\dots,S_r\}$, \citet{liang2005generalized} %consistently
estimated the integral $\int_S q(\omega)d\omega$ by  $\hat{g}(S)/\hat{g}(S_{1})$. Assuming convergence of GWL, a consistent estimate of $\lambda$ is thus given by $\hat{\lambda}_{GWL}=\log(\sum_{i=2}^r\hat{g}(S_i)/\hat{g}(S_{1}))$.

The key strengths of GWL are its adaptive nature and that it exhibits good mixing properties even for multi-modal targets, the latter property being a benefit of asymptotic uniform sampling across energy bins. In practice, a limitation of the algorithm  is that  the MSE of $\hat{\lambda}_{GWL}$ is bounded below for fixed $n_0$ and the specified geometric growth in $n_t$, as can be seen in the top left panel of Figure \ref{gwl_results} (discussed in Section \ref{sec:gwl_results}). (\citet{liang2007stochastic} attempted to mitigate this phenomenon, but the convergence properties of the updated algorithm again may not be ideal, and further developments are still being made; see for example \citet{jacob2014wang}.) Here we simply view GWL as a related method to compare against and combine with. For these purposes the lower bound on the convergence of $\hat{\lambda}_{GWL}$  does not play a large role because the number of target evaluations we allow is approximately equal to or lower than the number required by GWL to achieve its minimum MSE.
For further details of GWL the reader is referred to \citet{liang2005generalized}, \citet{liang2007stochastic},  \citet{bornn2013adaptive}, and \citet{jacob2014wang}.


\subsection{Combining GWL with Warp-U}\label{sec:gwl+warpu}

%We now consider the situation where GWL has been run for 10 stages, we think it is near convergence, and we can decide  whether to use the computation needed for an eleventh stage to continue running the algorithm (GWL-only) or to instead make use of Warp-U bridge sampling  to obtain $\hat{\lambda}^{\pU}_{\opt}$ (GWL+Warp-U). Draws from $p$ are required to implement the latter, but samples can be obtained from the first 10 stages of the GWL run without any additional target evaluations. In particular, to obtain a sample approximately from $p$ we first sample $k$ from $1,\dots,r$ according to the weights $w_i=\hat{g}(S_i)/\sum_{j=1}^r\hat{g}(S_j)$, for $i=1,\dots,r$, and then uniformly select one of the samples in subregion $S_k$ recorded during the first 10 stages of GWL. Since these samples require no new target evaluations, the only  new target evaluations required for Warp-U bridge sampling is the $mK$  needed to evaluate $\tilde{p}$ at the $m$ samples from $\phi$.

Consider a situation where GWL has been run for $T^* < T$ stages. We suspect that it is near convergence, and want to determine if we can reduce the MSE by using the computation to only complete the remaining $T-T^*$ stages (the GWL-only approach) or to make the use of Warp-U bridge sampling to obtain the estimator $\hat{\lambda}^{\pU}_{\opt}$ (the GWL+Warp approach). Draws from our target $p$ are required to implement the latter approach, but can be obtained from the GWL run without any additional target evaluations. To see this, first let $G_i$ denote the set of samples collected from subregion $S_i$ during the $T^*$ stages of the GWL run, for $i=1,\dots,r$.  With this notation, we propose the following addition to GWL.
\vspace{0.2cm}

\noindent{\bf Warp-U Addition.}
\noindent
\vspace{-\topsep}
\begin{enumerate}
\setlength{\itemsep}{-0.3cm}
\item For $l=1,\dots,n$, repeat the following two steps:
\vspace{-\topsep}
    \begin{enumerate}[(i)]
\setlength{\itemsep}{-0.3cm}
    \item Sample a subregion index $k\in\{2,\dots,r\}$ using the probabilities $b_i \propto \hat{g}(S_i)1_{\{G_i\not=\emptyset\}}$, for $i=2,\dots,r$.\\\vspace{-0.3cm}
    \item With uniform sampling, select a sample $\omega_l \in G_k$, i.e., select  one of the samples in subregion $S_k$ collected by GWL. \\\vspace{-0.3cm}
\end{enumerate}
    \item Apply Warp-U bridge sampling with $\{\omega_1,\dots,\omega_n\}$ and $m$ draws from $\phi$ to obtain the estimate $\hat{\lambda}^{\pU}_{\opt}$.
\end{enumerate}
The first step obtains draws from $p$ restricted to $\bigcup_{i=2}^rS_i$, and the second step applies Warp-U bridge sampling using these draws. The indicator $1_{\{G_i\not=\emptyset\}}$ in $b_i$ indicates that
we sample only  regions from which there are samples during the GWL run. %When this Warp-U addition is run after GWL we refer to the whole algorithm as the {\it GWL+Warp-U} approach, and if it is not run then we refer to the algorithm as the {\it GWL-only} approach.
Since $q(\omega_l)$, for $l=1,\dots,n$, has already been evaluated during the GWL run, the only  new target evaluations required for the above Warp-U addition are the $mK$  needed to evaluate $\tilde{q}$ at the $m$ draws from $\phi$. In step 2 above, we could alternatively apply standard bridge sampling to $p$ and $\phi_{\mix}$ to obtain $\hat{\lambda}^{\mix}_{\opt}$, as described in Section \ref{subsection::simulation_known_mixture}. We refer to this alternative approach as GWL+BS.

\subsection{Illustration of the GWL+Warp-U algorithm}
\label{sec:gwl_results}

We consider the 25 skewed-{\it t} mixture example from Section \ref{adaptive_bias}. We run the GWL-only algorithm for $T=25$ stages, and again set $\delta_0=e-1$. We try $n_0=10^3,10^4,10^5$ and find that larger $n_0$ requires more stages for the estimator $\hat{\lambda}_{GWL}$ to converge but leads to lower RMSE; see the top left panel of Figure \ref{gwl_results}. %The total number of target evaluations across the 25 stages  for these values of $n_0$ are approximately $10^5$, $10^6$, and $10^7$, respectively.
We choose $n_0=10^4$ as a compromise between RMSE and computational cost. The value of $n_0$ is not the target of our comparisons, nor is the choice of the proposal density $h$ or the partition $S_1,\dots, S_r$. We therefore
use our knowledge of the true target $p$ to configure these components to favor the GWL-only algorithm; see Appendix \ref{app:gwl_details} for details.

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.9\textwidth,trim=0mm 5mm 0mm 0mm,clip]{stage10_104_all_results.pdf}
%\caption{Graphical illustration of Warp-II and Warp-III transformation.}
\caption{\label{gwl_results}\small {The top left panel shows the RMSE of $\hat{\lambda}_{GWL}$ at each of 25 stages, for $n_0=10^3,10^4,10^5$. The solid lines indicate the results for 11-stage, 9-stage, and 5-stage runs of the GWL-only algorithm with $n_0=10^4$. The top right panel shows the RMSE of the GWL+Warp-U estimator (hollow symbols) and the GWL+BS estimator (solid symbols), where the initial GWL run is for 10 stages. The number of target evaluations used by the Warp-U or ordinary bridge sampling step is given on the {\it x}-axis as a  proportion of the target evaluations that would be needed for an eleventh stage of GWL (on a $\log_{10}$ scale). The different shapes correspond to different settings of $K$. %The solid horizontal line shows the $\log_{10}$ MSE when the GWL is run for 11 stages. All results are based on 100 repetitions and the corresponding uncertainties are relatively small.
The bottom left and right panels show similar results where the initial GWL run is for 8 and 4 stages, respectively. }}
\end{center}\end{figure}



%The left panel of Figure \ref{gwl_results} shows $\log_{10}$ of the mean squared error (MSE) for GWL estimator of the normalizing constant of $p$ (the true value is 1) at each of the 25 stages. The {\it x}-axis shows $\log_{10}$ of the cumulative number of target evaluations used. The dotted and dashed lines indicate the results at stage 4 and stage 5. These results are based on 100 runs of the algorithm.

The solid lines in the top left panel of Figure \ref{gwl_results} indicate the RMSE when the GWL-only algorithm (with $n=10^4$) is run for 5, 9, and 11 stages, and we see the RMSE is stabilized after stage 9. For reference, the same three RMSE values are indicated by a horizontal line in the top right, bottom left, and bottom right panels of  Figure \ref{gwl_results}, respectively. Running GWL for more than 9 stages does not improve the RMSE, but we can improve it using the Warp-U Addition detailed in Section \ref{sec:gwl+warpu}, even if we do not increase the overall computational cost. In the top right panel of Figure \ref{gwl_results}, the hollow symbols show the RMSE for the GWL+Warp-U estimator $\hat{\lambda}^{\pU}_{\opt}$, in the case where the GWL component was run for only 10 stages, thereby saving the computation needed for an $11^{\text{th}}$ stage to be used for Warp-U sampling.  Of course, we may decide we do not need to use all of the saved computation. The $x$-axis of Figure \ref{gwl_results} gives the number of target evaluations we use for the Warp-U step, in units of $\log_{10}$ of the proportion of target evaluations needed for an $11^{\text{th}}$ stage of GWL, i.e., at $0$ on the $x$-axis the computational cost of the Warp-U sampling matches that of an $11^{\text{th}}$ stage. The different hollow shapes correspond to different values of $K$ (number of mixture components). For comparison, the horizontal line indicates the RMSE under the GWL-only algorithm after 11 stages (for which the $x$-axis is irrelevant). At $0$ on the $x$-axis the GWL-only and GWL+Warp-U methods use the same number of target evaluations, but the GWL+Warp-U method yields substantially lower RMSE for all four values of $K$ (2, 5, 10, and 20). Indeed, the RMSE obtained is even lower than that achieved by the GWL-only algorithm with $n_0=10^5$ after 11 (or 25) stages, which uses a factor of 10 more target evaluations than used by the  GWL+Warp-U runs (with $n_0=10^4$). %When we apply Warp-U with only half the number of target evaluations needed for an eleventh stage of GWL (around $-0.3$ on the {\it x}-axis) we still see a large reduction in RMSE compared with running an eleventh stage.
This example suggests that applying Warp-U when GWL is at or close to convergence offers a way to substantially lower RMSE with only the number of target evaluations required to run one more stage of GWL (or even fewer). The improvements offered by GWL+Warp-U are thus almost free because we can stop GWL one stage early, and in any case the number of target evaluations required by the Warp-U part is relatively low. %Even if the Warp-U part is viewed as extra computation, the number of target evaluations it requires is relatively low compared with the total number used by GWL.

%Even for the case where only a tenth of the target evaluations needed for a fifth stage of GWL are used ($-1$ on the {\it x}-axis), GWL+Warp-U still offers large improvements over the GWL only mention for $K=5,10,20$.

For further comparison, the solid shapes in the top right panel of Figure \ref{gwl_results} show results for the GWL+BS method, i.e, where the two bridge sampling densities are $p$ and $\phi_{\mix}$. Note that, at any given point on the {\it x}-axis the number of target evaluations is the same for the GWL+BS and GWL+Warp-U algorithms, which is achieved by setting $m=n(2K-1)$ in the GWL+BS algorithm and $m=n$ in the GWL+Warp-U algorithm. We see that GWL+BS again achieves substantially lower RMSE than is obtained by simply running an $11^{\text{th}}$ stage of the GWL-only algorithm. The RMSE under the GWL+BS method is also seen to be marginally lower than that under the GWL+Warp-U method, but now that we have controlled the number of target evaluations, we see the performance is very similar. % For a shorter initial run of GWL (bottom right panel of Figure \ref{gwl_results}) we see that     However, the MSE under the GWL+BS method is always higher than that under the GWL+Warp-U approach, again illustrating the additional gains made possible by the Warp-U transformation in the context of multi-modal $p$.

Naturally, Warp-U or standard bridge sampling can be applied after any number of GWL stages; we do not have to wait until we are sure of convergence. To investigate this, we ran the GWL+Warp-U and GWL+BS algorithms again but where the initial GWL run was shorter. The bottom left and bottom right panel of Figure \ref{gwl_results} show results in the case where the initial GWL run was 8 and 4 stages, respectively. These results are qualitatively similar to before, except that GWL+Warp-U occasionally performs slightly better than GWL+BS (e.g., when $K=5$ in the bottom right panel).  The main constraint on when Warp-U or standard bridge sampling can be used is that GWL needs to have been run for long enough to have explored regions where $p$ has high density.  Otherwise, weighted re-sampling of the GWL samples will not yield approximate draws from $p$. This is not a major issue in practice because, % neither GWL or any method that uses its output is likely to produce a good normalizing constant estimate if $p$ has not been properly explored.
as can be seen in the top left panel of Figure \ref{gwl_results}, GWL substantially reduces RMSE in its initial stages, and it is likely to be the latter stages where applying Warp-U or standard bridge sampling is  most appealing.




==> sec6.tex <==
\section{Strategies for Making Further Improvements}
\label{sec:discussion}


We have seen that stochastic Warp-U transformations can transform a multi-modal density $q$ into an approximate Normal density (or some other convenient auxiliary density $\phi$). The transformed density $\tilde{q}$ has the same normalizing constant $c$ as the original target density $q$. Furthermore, since the overlap between $\tilde{q}$ and the base density $\phi$ is typically large, performing bridge sampling with the transformed draws $\{\tilde{\omega}_1,\dots,\tilde{\omega}_n\}$ produces an accurate estimate of $c$. In particular, Theorem 1 implies that the accuracy is equal to or greater than that obtained if we perform bridge sampling using the original draws $\{\omega_1,\dots,\omega_n\}$ and the densities $q$ and $\phi_\mix$. Thus, in terms of statistical efficiency, Warp-U transformations are always beneficial, especially when the target density is multi-modal. However, there are still a number of important directions for further developments, especially regarding computational efficiency and identifying a good approximating mixture distribution $\phi_{\mix}$, which we now discuss. % We now discuss these opportunities for further work.

\subsection{Reducing the Cost of Transformed Density Evaluations}

From (\ref{equ::Warp-U-transformed-density}), it is seen that the density $\tilde{q}$ is at least $K$ times more expensive to evaluate than $q$. Consequently, in Figure \ref{gwl_results} we saw that despite its greater statistical efficiency, Warp-U bridge sampling performs similarly to ordinary bridge sampling with  $q$ and $\phi_\mix$, after accounting for the number of target evaluations needed, i.e., evaluations of $q$.  %In practice, the case of expensive $q$ evaluations is of most interest, but in other situations where $q$ is not expensive enough to dominate the computational cost, %In Figure in Section we saw that when $q$ is not expensive enough to dominate computational cost, then the   in some cases the precision per second The most important case in practice is when $q$ is
When evaluating $q$ is inexpensive, ordinary bridge sampling can perform substantially better than Warp-U bridge sampling, in terms of precision per CPU second, e.g., see Figure \ref{fig::50D_PpS_156}. The greater efficiency of ordinary bridge sampling in such cases is due to the many multivariate Normal evaluations required by Warp-U bridge sampling. These evaluations are not prohibitively expensive and in practice will often be of secondary concern to $q$ evaluations. Cases where $q$ is inexpensive to evaluate  are generally of less interest because many methods will be practical in this scenario. Thus, we are primarily concerned with the statistical efficiency of Warp-U as a function of $q$ evaluations.

We therefore need to find ways to reduce the computational cost of evaluating $\tilde{q}$.
Direct density approximation is unlikely to be fruitful in high dimensions. A plausible strategy is to randomly select only some of the $K$ terms in (\ref{equ::Warp-U-transformed-density}) to evaluate, as is done in the mixture sampling method of \citet{elvira2019generalized}; they randomly partitioned the set of sampling densities and then used these partitions in computing importance weights. Specifically, the importance weight for a sample $\omega$ drawn from density $p_s$ is set to be  the reciprocal of the average of the sampling densities in the same partition as $p_s$. % the true density that $\omega$ was drawn from. as the true  single partition when computing each importance weight. %  for reducing the computational cost of Warp-U sampling is to approximate the density $\tilde{q}(\tilde{w};\bz)$ in (\ref{equ::Warp-U-transformed-density}).
We could apply a similar approach by viewing the terms $c\tilde{p}^{(k)}(\tilde{\omega})=cp^{(k)}(S_k\tilde{\omega}+\mu_k)$) in (\ref{equ::Warp-U-transformed-density})  as the weighted and unnormalized sampling densities.
However, we do not know from which weighted component $c\tilde{p}^{(k)}$ each sample $\tilde{\omega}\sim \tilde{p}$ originated. Furthermore, the $c\tilde{p}^{(k)}$ incorporate unknown weights, so the unweighted mixture components of $\tilde{q}$ are not available and therefore we cannot weight them by their empirical weights, as is required by (generalized) bridge sampling, e.g., the weights $s_i$, for $i=1,2$, in (\ref{optestimator}).  Regarding the unknown sampling component $c\tilde{p}^{(k)}$, it may be sufficient to stochastically impute  the index of the ``true"  component  by drawing  from the conditional distribution $\varpi(\Psi|\omega)$ in (\ref{equ::varpi_theta_omega}). A possible solution to the second difficulty is to use the theoretical component weights incorporated in the $c\tilde{p}^{(k)}$ in the final bridge sampling estimator as opposed to the observed weights. In summary, there are feasible methods for improving the computational efficiency of Warp-U bridge sampling,  but the several potential strategies need to be further explored. %, including the use of a better adapted reference density, discussed below.

%In addition to increasing computational efficiency, it is also of interest to simply reduce computation time which is likely possible through parallel computation. Bridge sampling with the  Warp-U transformed data is embarrassingly parallelizable, because each sample can be treated individually until the final computation of (\ref{optestimator}).
%If a large number of nodes are available then the bottleneck may in fact be the estimation of $\bz$ via the EM algorithm. Thus, a parallel version of EM or a clustering method, such as the $k$-means algorithm, could be especially effective in reducing the computation time of Warp-U bridge sampling estimators.


\subsection{Base and Mixture Distribution Selection}
\label{sec:base_and_mle}

So far we have focused on using the standard Normal as the base distribution $\phi$. But
Theorem 1 implies that
the $f$-divergence between $(\phi_\mix, p)$ is larger than that between $(\phi,\widetilde{p})$ for {\it any} continuous densities $p$ and $\phi$.
For heavy-tailed targets, using a {\it t}-distribution may be more effective for capturing
the mass of $p$, that is, a {\it t}-density may allow us to use a mixture $\phi_{\mix}$ with fewer components and thereby reduce computational costs.
In other contexts, the support of $p$ may be bounded and then a base density with bounded support would be more appropriate. Perhaps in some scenarios it would make sense for $\phi_{\mix}$ to be a mixture of several different base densities, in which case some modifications to the development here would be needed. With a different choice of the base function, a different method for fitting $\phi_{\mix}$ would be required, e.g.,  for the {\it t}-distribution, we could use the approach of  \citet{peel2000robust} to fit $\phi_{\mix}$.
%Nonetheless, we suggest using the diagonal covariance matrix for the components in $\phi_\mix$ and
%using our strategy in Figure \ref{fig::solution_small_bias_variance} to remove the adaptive bias.
%

Secondly, although our approach for fitting the Warp-U parameters  $\bz$ is promising in practice, it is almost certainly not optimal. \citet{kong2003theory} showed that a standard bridge sampling estimator is in fact a maximum likelihood estimator (MLE), and it may be possible to use the same likelihood framework to find an optimal estimator for $\bz$.
More specifically, let $\phi_i$
be the pdf of $\Normal(\mu_i, \Sigma_i)$, for $i=1,\ldots, K$, and
$\phi_\mix=\sum_{i=1}^K\pi_i\phi_i$. %,
%$n_i$ be the number of draws from $\phi_i$, and $m=\sum_{i=1}^Kn_i$.
Then the maximum likelihood estimator of $c$ (with $p=q/c$ as before) identified by  \citet{kong2003theory} is \begin{equation}
\hat{c} = \sum_{i=1}^2\sum_{j=1}^{n_i}\frac{q(w_{i,j})}{n_1\hat{c}^{-1}q(w_{i,j})+n_2\phi_{\mix}(\omega_{i,j})},\label{eqn:mle}
\end{equation}
where $\{\omega_{1,1},\dots,\omega_{1,n_1}\}$ are draws from $p$, and $\{\omega_{2,1},\dots,\omega_{2,n_2}\}$ are draws from $\phi_{\mix}$.
%When  $n_i/m\rightarrow\pi_i$,
The estimator (\ref{eqn:mle}) is the same as  $\hat{c}_{\opt}^{\pmix}=\exp(\hat{\lambda}_{\opt}^{\pmix})$. %The estimator (\ref{eqn:mle}) is derived from a likelihood that treats the baseline measure $\measure(\ud\omega)$ as the unknown, which is natural considering that all integral estimators approximate the baseline measure in some way. \citet{kong2003theory} and \citet{kong2007further} build on this by showing that statistical efficiency  can be further improved, at the cost of computation, by enforcing (true) invariances of $\measure(\ud\omega)$ under selective transformations of $\omega$.
If Warp-U transformations can be correctly incorporated into this likelihood framework then we can use the MLE of $(c,\bz)$ to improve upon our current approach. %\citet{jones_qualifying} provides further insights on how this likelihood formulation might be achieved and identifies some open challenges.  
Whether using a maximum likelihood approach or not, it is especially important to investigate further how the number of components $K$ should be chosen.

\subsection{It's Time to Build a Bridge}
The vast majority of the MC literature is about improving MC \textit{sampling} efficiency, that is, how to design MC sampling algorithms most effectively. In contrast,  bridge sampling, with or without warp transformations, is about improving MC \textit{inference} efficiency, that is, how to gain more precision with a given set of MC draws. Adding warp bridge sampling to GWL provides an example of bridging the sampling and analysis approaches, a strategy we believe has much more to offer than the current literature recognizes.  We therefore invite interested readers to join us in laying further foundations for this much needed bridge.


\begin{comment}
Whether using a maximum likelihood approach or another method, it is especially important to investigate further how the number of components $K$ should be chosen.
When $K$ is small compared with $n$, both the computational costs and the statistical efficiency of the Warp-U bridge sampling estimator increase with $K$, as shown in the simulation studies in Appendix
\ref{app:tuning}. However, we find that $K$ should be $\leqslant n/100$, because when $K>n/100$, the mixture model will overfit the data (i.e., the draws from $p$) and the resulting $\phi_{\mix}$ density does not have more overlap with $p$ than when $K=n/100$. While this is a useful starting point, in practice, it would be helpful to have detailed guidance that more precisely balances computational cost and statistical efficiency. Generally, we can get a good estimate of the computational cost as a function of $K$, but it is difficult to estimate how the MSE
of the estimator changes with $K$.
Some widely-used criteria, such as AIC and BIC, deal with the trade-off between the
goodness-of-fit of a model and its complexity, and may be useful for our purpose.
But it is not immediately clear that these generic model considerations properly capture the statistical and computational
efficiency of Warp-U bridge sampling.
Another method, perhaps better suited to our purpose, was  proposed by
\citet{lee2006estimating} and estimates the optimal $K$ for a mixture by dynamically adding components one by
one based on an incremental $k$-means algorithm until some specific criteria are met. %Greater statistical efficiency  with only moderate increases in computation could potentially be achieved by a version of Warp-U bridge sampling that uses this approach provided that, whenever a component is added, we can somehow reuse the computation from the previous value of $K$.
\end{comment}




%There are  more questions we have not explored.
%Theorem 1 states $\mathcal{D}(\widetilde{p},\phi)\leqslant \mathcal{D}(p,\phi_{\mix})$ for any increasing function of the $f$-divergence.
%However, we have little knowledge about  the amount of reduction in the divergence, and
%when the superiority of $\hat{\lambda}_\alpha^\pU$ to $\hat{\lambda}_\alpha^\pmix$ is more evident in terms of the statistical efficiency.
%In addition, we have not investigated how the dependence of the data would affect our algorithm.
%We would also like to explore more applications of the Warp-U transformation.
%%, possibly in the areas of calculating expectations and sampling,  like the importance sampling method.
%




